Fantastic Rewards and How to Tame Them: A Case Study on Reward Learning for Task-oriented Dialogue Systems

When learning task-oriented dialogue (ToD) agents, reinforcement learning (RL) techniques can naturally be utilized to train dialogue strategies to achieve user-specific goals. Prior works mainly focus on adopting advanced RL techniques to train the ToD agents, while the design of the reward function is not well studied. This paper aims at answering the question of how to efficiently learn and leverage a reward function for training end-to-end (E2E) ToD agents. Specifically, we introduce two generalized objectives for reward-function learning, inspired by the classical learning-to-rank literature. Further, we utilize the learned reward function to guide the training of the E2E ToD agent. With the proposed techniques, we achieve competitive results on the E2E response-generation task on the Multiwoz 2.0 dataset. Source code and checkpoints are publicly released at https://github.com/Shentao-YANG/Fantastic_Reward_ICLR2023.

==> Reward Learning for Dialogs (ICLR 2023)/Tex/Background.tex <==
\vspace{-.2em}
\section{Background} \label{sec:background}
\vspace{-.2em}
%------------------
% Out
%
%-------------------

\myparagraph{Task-oriented dialogue as reinforcement learning.} \label{sec:tod_rl}
We formulate the problem of the ToD system as a partially observable Markov decision process (POMDP) \citep{kaelbling1998planning}, 
specified by $\gM = \langle \sS, \sA, \sO, \gP, \gR, \gamma\rangle $, where state $s \in \sS$ consists of the previous dialogue history $h$ and the user intended goal $g$ specified prior to the start of the dialogue; 
$o \in \sO$ is the observation that can be the user utterance; action $a \in \sA$ can be the system response or dialogue act; %, whose dimension is the size of the whole vocabulary (denoted by $|\sA|$);
$\gP(s^\prime \given s, a)$ is the underlying transition probability; 
$\gR(h, a, g)$ is the intermediate reward function for taking action $a$ under dialogue history $h$  and goal $g$; and $\gamma \in [0, 1]$ is the discount factor.

The dialogue history $h_t$ at timestep $t$ consists of all the previous observations and actions, \ie, $h_t \triangleq \{o_0, a_0,\ldots, o_{t-1}, a_{t-1}, o_t\}$. 
Since the ToD agent cannot directly observe the user goal $g$, it makes a decision based on the entire dialogue history $h_t$ so far.
Specifically, the policy $\pi$ is defined as a mapping from $h_t$ to a probability distribution over $\sA$, \ie, $\pi \triangleq \pi(a_t \given h_t)$.
The training objective is to find a policy $\pi$ that maximizes the expected (discounted) cumulative reward
\begin{align*}\textstyle
    J(\pi) \triangleq \E_{\mu_{g}, \pi, \gP}\left[\sum_{t=0}^{T}\gamma^t \gR(h_t, a_t, g)\right]\,,
\end{align*}
where $\mu_{g}$ is the distribution of goals and $T$ is the number of turns in the dialogue trajectory.
% %%%%%
% When the policy $\pi_{\theta}$ is parameterized with $\theta$, we can optimize $\theta$ by taking one step ascent with policy gradient \citep{rlintro2018}:
% \begin{align}
%     \nabla_{\theta}J(\theta):= \E
% \end{align}
%%%%%%%


\myparagraph{Reward design and learning in ToD systems.}%\label{sec:rew_from_pref}
Unlike the classical RL problems where the intermediate reward function is well designed and provided,
in ToD systems we can only get the evaluation results at the end of the dialogue \citep{multiwoz2018}.
Consequently, most of the existing works adopt the manually designed intermediate reward function that only gives binary reward to indicate whether the dialogue agent achieves the goal or not \citep[\eg,][]{weisz2018sample,wu2019switch,gptcritic2022}:
\begin{align*}\textstyle
 \gR(h_t, a_t, g)= \begin{cases}
     ~~~R_\mathrm{const}~~\text{or}~~0, & \text{if goal}~g~\text{is achieved at timestep}~t \,,\\ 
     -R_\mathrm{const}, & \text{if goal}~g~ \text{is not achieved at timestep}~t\,,
 \end{cases}
\end{align*}
where $R_\mathrm{const}$ is a positive constant that can be 1.
However, such a sparse reward signal can be one of the reasons that the ToD agents from RL often have poor performance \citep{takanobu2019guided,wang2020learning}.
A similar issue is also observed in goal-oriented RL \citep{andrychowicz2017hindsight}. 
%\st{is this sparse? it has value at every timestep? YF: this is definition of sparse reward RL, you can check HER. }

To address the above issue, a few recent works focus on learning an intermediate reward function from demonstrations or mechanical dialogue assessments \citep[\eg,][]{wang2020learning,caspi2021}, inspired by the reward-learning-from-preferences in RL \citep[\eg,][]{christiano2017deep,trex2019,drex2020}.
% Unlike traditional RL where the dense reward function is well defined and provided, 
% in most ToD system, one can only assess the entire dialogue history $h_T$.
% To apply RL to train ToD system, it is thus necessary to learn a parameterized per-turn reward function $\hat r\br{h_t, a_t,g;\theta}$ from the dialogue-level assessments, which is similar to reward learning from preference in imitation learning (IL).
More precisely, suppose we are given two dialogue trajectories $\tau_i$ and $\tau_j$, taking the form $\tau_i\triangleq\{g^{(i)}, (o_0^{(i)}, a_0^{(i)}),\ldots,(o_T^{(i)}, a_T^{(i)})\}$.
We want to learn a parametrized reward function $\gR_{\theta}(o_t, a_t, g)$ with parameter $\theta$,\footnote{We use the belief state, action, and goal as the reward function inputs. 
The belief state is part of the observation $o_t$. We also drop the dependency on $h_t$ for $\gR_{\theta}$ to simplify the reward function learning.} such that
$\sum_{t=0}^{T}\gR_{\theta}(o_t^{(i)}, a_t^{(i)}, g^{(i)}) > \sum_{t=0}^{T}\gR_{\theta}(o_t^{(j)}, a_t^{(j)}, g^{(j)})$ when $\tau_i$ is preferred over $\tau_j$ (denoted as $\tau_i \succ \tau_j$) and \textit{vice versa}. 
Then one can follow the  Bradley-Terry model of pairwise preferences \citep{bradley1952rank} to train the reward function by minimizing the loss
\begin{equation}\label{eq:original_pref_rew}\textstyle
\resizebox{.63\linewidth}{!}{%
$
    \ell(\theta) = -\sum_{\tau_i \succ \tau_j}\log \sbr{ \frac{\exp\br{\sum_{t=0}^{T}\gR_{\theta}(o_t^{(i)}, a_t^{(i)}, g^{(i)}) }}{\sum_{k \in \{i, j\}}\exp\br{\sum_{t=0}^{T}\gR_{\theta}(o_t^{(k)}, a_t^{(k)}, g^{(k)})} } }\,.
    $%    
}
\end{equation}
$\ell(\theta)$ can be interpreted as a pairwise ranking loss, which is formalized as binary classification in the problem of learning to rank \citep{ranksvm1999,rankingboosting2003,ranknet2005}.
%In the classical IL approach \citep[\eg,][]{christiano2017deep,trex2019,drex2020}, one assume pairwise preferences on trajectories in the dataset. 
%Denote $h_T^i \prec h_T^j$ if dialogue trajectory $h_T^j$ is preferred over trajectory $h_T^i$.
%The reward function $\hat r\br{h_t, a_t,g;\theta}$ is trained by following the Bradley-Terry model of preferences \citep{bradley1952rank} and by assuming that the preferences result from the sum of rewards of each trajectory. 
%where $\abs{\gD}$ is the size of the dataset, $g^j$ and $g^i$ are respectively the goal of trajectory $h_T^j$ and $h_T^i$.

% \myparagraph{End-to-End Task-Oriented Dialogue Systems.}
% Task-Oriented dialogue systems are designed to achieve a goal specified by a user in natural language.
% The classical approach to solve this problem usually requires solving several sub-tasks \citep{williams2007partially,gao2018neural}, including 
% More recently, as a way to simplify the system design and reduce human supervision, end-to-end models for the task-oriented dialogue system \citep[\eg,][]{mintl2020,simpletod2020,soloist2021} were proposed,
% some of which significantly improve the overall performance by leveraging the pre-trained language models \citep[\eg,][]{devlin2018bert,radford2019language,bart2019}. 
%   such as MinTL \citep{mintl2020}, to , without changing the underlying structures of the original training frameworks. \jg{Maybe you can put the last sentence into related work.} 
%utilized to guide the training of response-generation model, which provides an enhancement to the original end-to-end training frameworks such as MinTL \citep{mintl2020}, without changing the underlying structures. 

%As an illustration to demonstration our proposed reward-learning approach, we build our framework on MinTL \citep{mintl2020}, with a pre-trained language model BART \citep{bart2019} as the backbone. \st{Already (and better) say this in the experiment section?}








==> Reward Learning for Dialogs (ICLR 2023)/Tex/Intro.tex <==
\vspace{-.4em}
\section{Introduction}\label{sec:intro}
\vspace{-.4em}


% Outlines
%------------------
% dialog as end-to-end, supervised, it can also be viewed as RL
% 2. issue with the problem as RL 
% 3. proposal in this paper (mimic context awareness)
%-----------------
% Example: Task-oriented dialogue (TOD) systems, which interact with the users in multiple turns via natural languages to accomplish tasks such as weather inquiry, ticket booking or schedule planning, play important roles in daily life\citep{chen2017survey,kwan2022survey}.  
% Traditionally, the problem of ToD is decomposed into several sub-tasks \citep{smith1994spoken,young2013pomdp}:
% natural language understanding (NLU),
% dialogue state tracking (DST),
% dialogue management (DM) 
% and natural language generation (NLG).
% This pipeline approach, however, requires intensive structural designs and comprehensive data annotation for training \citep{kwan2022survey}.

The bloom of pre-training language models \citep[\eg,][]{devlin2018bert,bart2019,radford2019language,zhang2022opt} have significantly pushed the boundaries of natural language processing (NLP) on real-world tasks.  
Among all the promising potentials, one important application is the task-oriented dialogue (ToD) systems, which interact with the users in multiple turns via natural languages to accomplish tasks such as weather inquiry, ticket booking, or schedule planning \citep{chen2017survey,kwan2022survey}.

Traditionally, the problem of ToD is decomposed into several sub-tasks \citep{smith1994spoken,young2013pomdp}:
natural language understanding (NLU) for understanding turn-level user intents or slot values \citep{tur2011spoken,casanueva2020efficient}, 
dialogue state tracking (DST)  for tracking user belief state across multiple dialogue turns \citep{zhang2019find,zhu2020convlab}, 
dialogue management (DM) for choosing system actions to take \citep{peng2017composite,zhao2019rethinking}, 
and natural language generation (NLG) for mapping system actions to natural language responses \citep{wen2015semantically,damd2020}.
This pipeline approach, however, requires intensive structural designs and comprehensive data annotation for model training \citep{kwan2022survey}.
Recently, there has been a growing interest in building end-to-end (E2E) ToD agents, which directly
generate responses based on the natural language conversation mixing user utterances and past responses.
%, without sub-tasking. 
% map from the user utterance and dialogue history to system response in natural languages, 
% \ky{rewrite? I don't get the gist of end-to-end here. Maybe sth like "directly generate responses conditioned on the natural language conversation mixing user input utterances and previous responses, without xxx".}.
Apart from this structural simplicity, many of the E2E ToD models can utilize the pre-trained language models and are simply trained by supervisedly fine-tuning the pre-trained models on the ToD datasets \citep[\eg,][]{simpletod2020,ham2020end,mintl2020,soloist2021}. 

Due to the intrinsic similarity between dialogues and sequential decision-making, reinforcement learning (RL) methods are naturally employed to train dialogue systems and have achieved some success \citep[\eg,][]{williams2007partially,georgila2011reinforcement,zhao2019rethinking}.
Since interacting with users during the training process is mostly impractical, offline RL \citep{batchrl2012,offlinetutorial2020}, \ie, RL on static datasets, has recently been adopted to train E2E ToD models \citep[\eg,][]{offlinerldialog2019,jaques2020human,caspi2021,snell2022offline,snell2022context,gptcritic2022}.
Although this direction already presents promising empirical results, an open question exists on how to properly design the reward function for the underlying (offline) RL.
Existing works \citep[\eg,][]{wu2019switch,gptcritic2022,snell2022context} manually design a sparse reward function that only indicates whether the agent achieves the goal or not.
Unfortunately, due to the delayed feedback, learning from such a sparse reward signal is itself challenging for RL agents \citep{andrychowicz2017hindsight,liu2018competitive,aim2021}. 
% \ky{since a complete conversation typically consists of multiple turns of generating responses}. \ky{Maybe also mention collecting one conversion is time-consuming given the wizard-of-oz approach, which the number of training data small? This indicates we need to use existing data more effectively and efficiently.  }
When applied to train the more complicated ToD agents, the sparse reward signal could lead to poor empirical performance \citep{takanobu2019guided,wang2020learning}. 
To address this issue, we aim at answering the following question in this~paper:
\begin{center}
    \vspace{-.28em}
    \textit{How to efficiently \textbf{learn} a reward function and \textbf{leverage} it for training E2E dialogue agents?}
    \vspace{-.28em}
\end{center}
We answer the \textit{first half of this question} by introducing two reward-learning objectives, \rewardnet and \texttt{RewardMLE}, based on the classical learning-to-rank literature \citep{listnet2007,listmle2008}. 
Our desiderata is a reward function that can ``explain" some non-trivial preference-based ordering among multiple alternative dialogue trajectories, thus potentially allowing the resulting RL-trained ToD agents to have better-than-demo performance.
We accomplish this goal by learning a parameterized reward function on dialogue turns, from which the accumulated reward of a dialogue trajectory can reflect the preference among multiple alternatives. 
We answer the \textit{second half of the question} by
utilizing the learned reward function to guide the training of the E2E ToD system, with special considerations on the training stability.
% by leveraging the learned reward function to provide a stable policy gradient method to guide the training of the end-to-end ToD agents.
With these answers to the above question, 
%Combining the proposed techniques on the training and utilization of the reward function, 
we % can utilize the proposed techniques to train end-to-end ToD agents, which can
achieve competitive results on the E2E response-generation task on the widely-used dialogue benchmark MultiWOZ 2.0 \citep{multiwoz2018}. 
Several ablation studies and analyses are conducted to provide further insights into the proposed techniques.
% \ky{can you use one sentence to link sparsity with poor performance? e.g, not effectively learning policy from each turn? } 

% GPT-Critic \citep{gptcritic2022} is one of the representative works, where the authors proposed to train an action-value (critic) function under the offline setting, and generate actions based on the critic values that can be further utilized for dialogue agent learning. 
% Though such direction seems to be promising, it still remains unknown how to design the reward function properly for ToD tasks.

% if no other technique such as relabelling \citep{andrychowicz2017hindsight} is considered to address the issue. 

%\yy{add some more discussion on reward design and learn to motivate, maybe some discussion on caspi}
% Besides, the common used pairwise preference loss  for reward learning \citep{christiano2017deep,trex2019} can be viewed as a special case of the \rewardnet loss \yy{maybe remove, not important?}.

==> Reward Learning for Dialogs (ICLR 2023)/Tex/conclusion.tex <==
\vspace{-.5em}
\section{Conclusion}
\vspace{-.5em}
In this paper, we aim to answer the question of how to efficiently learn and utilize a reward function for training the E2E ToD agents. 
We answer this question by introducing two generalized reward-learning objectives, and utilize a stable policy-gradient method to guide the training of the E2E ToD agents. 
%With the proposed techniques, we can achieve competitive results on the E2E dialogue task on the Multiwoz 2.0 dataset. 
Future work includes extending our reward-learning objectives to other applications, such as the question-answering with verification. 


==> Reward Learning for Dialogs (ICLR 2023)/Tex/experiments.tex <==
\vspace{-.4em}
\section{Experiments}\label{sec:exp}
\vspace{-.4em}

\myparagraph{Dataset.} 
We evaluate the proposed methods on the MultiWOZ 2.0 dataset \citep{multiwoz2018}, which is a representative ToD benchmark.
MultiWOZ 2.0 is a large-scale multi-domain dialogue corpus 
% consisting of conversations between a tourist/user and a clerk/system at an information center of a tourist city.
with seven domains:  attraction, hospital, police, hotel, restaurant, taxi, and train. Each dialogue therein covers between one to three domains.
This dataset has $8438$ dialogues in the training set and $1000$ dialogues in the validation and test set respectively.

\myparagraph{Evaluation Metrics.} 
Our proposed method is evaluated on the E2E dialogue-modeling task of the MultiWOZ 2.0 dataset.
Following the standard setup \citep[\eg,][]{multiwoz2018,sfnrl2019}, we use four automatic evaluations metrics:
1) \textbf{Inform} rate: the fraction of the dialogues where the system has provided an appropriate entity;
2) \textbf{Success} rate: the fraction of the dialogues where the system answered all the requested information;
3) \textbf{BLEU} score \citep{bleu2002}: measures the fluency of the generated responses;
4) \textbf{Combined Score} \citep{sfnrl2019}: an overall quality measure defined as $\mathrm{Combined~Score} =: (\mathrm{Inform} + \mathrm{Success}) \times 0.5 + \mathrm{BLEU}$.
% All our provided results are the average over five random seeds.
Details on prepossessing and implementation are in Appendix~\ref{sec:algo_box} and~\ref{sec:impl_details}.


\begin{savenotes}
\begin{table}[tb] 
\vspace{-2mm}
\captionsetup{font=small}
\caption{
\footnotesize{Results of the E2E response generation task on the MultiWOZ 2.0 dataset.
The best result on each metric is bold.
The results of UBAR are from the reproduction by \citet{gptcritic2022}.
The results of CASPI are from our reproduction.
All our provided results are the average over five random seeds.
Other results are from the original paper.
``GS" denotes the Gumbel-softmax trick.
$(\cdot)^{1}$ denotes the power function with power $1$.}
} 
\label{table:main} 
\vspace{-.7em}
\centering 
% \def\arraystretch{1.2}
% \setlength\tabcolsep{15pt}
\resizebox{.70\textwidth}{!}{
\begin{tabular}{@{}lcccc@{}}
\toprule
Algorithms                                           & Inform & Success & BLEU  & Combined Score \\ \midrule
SFN + RL    \citep{sfnrl2019}                                           & 73.80  & 53.60   & 16.90 & 83.10          \\
DAMD       \citep{damd2020}                                          & 76.40  & 64.35   & 17.96 & 88.34          \\
SimpleTOD \citep{simpletod2020} & 84.40  & 70.10   & 15.01 & 92.26          \\
MinTL     \citep{mintl2020}                                           & 84.88  & 74.91   & 17.89 & 97.78          \\
SOLOIST  \citep{soloist2021}                                            & 85.50  & 72.90   & 16.54 & 95.74          \\
UBAR \citep{ubar2021}                                                & 87.47  & 74.43   & 17.61 & 98.56          \\
GPT-Critic  \citep{gptcritic2022}                                         & 90.07  & 76.63   & 17.83 & 101.13         \\
CASPI\footnote{
The CASPI paper reports the median score over random seeds, instead of the more commonly used mean score.
We run the official CASPI codebase (\href{https://github.com/salesforce/CASPI}{https://github.com/salesforce/CASPI}) and report the mean scores.
}  \citep{caspi2021}                                              & 91.37  & 82.80   & 17.70 & 104.78         \\ 
\midrule
\texttt{RewardNet}, $N=3$, $\Phi=(\cdot)^{1}$ & 92.77 & 84.28 & 17.74 & 106.27 \\
\texttt{RewardMLE}, $N=5$, $\Phi=\exp(\cdot)$ & 91.49 & 83.38 & \textbf{18.97} & 106.40 \\
\texttt{RewardNet} + GS, $N=3$, $\Phi=(\cdot)^{1}$ & 92.63 & \textbf{84.32} & 18.35 & \textbf{106.83} \\
\texttt{RewardMLE} + GS, $N=5$, $\Phi=\exp(\cdot)$ & \textbf{93.09} & 83.90 & 18.04 & 106.54 \\
\bottomrule
\end{tabular}
}
\vspace{-1.5em}
\end{table}
\end{savenotes}

\vspace{-.4em}
\subsection{Main Results} \label{sec:exp_main} 
\vspace{-.4em}



\myparagraph{Main evaluation.} 
Table~\ref{table:main} compares the performance of our methods with several classical and recent approaches in the E2E response-generation task.
% outperforms baselines: good inform and success and good bleu score
As shown in Table~\ref{table:main}, our proposed methods not only improve the dialogue-task completion, measured by the Inform rate and the Success rate; but also generate fluent responses, reflected by the competitive BLEU scores.
% compare with CASPI (special case), 
Recall that CASPI is a special case of the \texttt{RewardNet} loss (Eq.~\eqref{eq:listnet}) when we use escort transform ($\Phi = (\cdot)^{1}$, the identity function) with pairwise preference ($N=2$).
%our proposed method when using the pairwise version of the ListNet loss and when the probabilistic transform in Eq.~\eqref{eq:listnet} is the escort transform with power one.
% using listwise ranking improve score (w. simple why?)
When we use three dialogue trajectories ($N=3$) to construct the \texttt{RewardNet} loss and retain the same escort transform, the overall performance generally improves over CASPI.
As discussed in \Secref{sec:main_rew_obj}, our \rewardnet loss generalizes the pairwise-preference learning by taking more information on each update of the reward model and thus could learn a better reward function.
Appendix~\ref{sec:detailed_comp_caspi} further compares our methods with CASPI.

% using listmle improves performances since it is more robust to the error in scores
The performance is further gently improved by changing the \rewardnet loss (Eq.~\eqref{eq:listnet}) to the \rewardmle loss (Eq.~\eqref{eq:listmle}), with the softmax transform ($\Phi = \exp(\cdot)$) and $N=5$ dialogue trajectories.
This again demonstrates the benefit of our proposal of using multiple trajectories to learn the reward model. \Secref{sec:exp_abla} conducts ablation studies on the number of trajectories and choice of $\Phi$.
% This gain may come from the relative robustness of the RewardMLE loss to small errors in the scoring process since the RewardMLE loss only uses the ranking of the provided scores, but not the numerical score values as in the RewardNet loss.

% Adding GS to both models further improve scores: directly optimize the learned reward func. is effective
So far, we follow the prior work to not utilize policy gradient to train the response-generation model, \ie, $\alpha=0$ in Eq.~\eqref{eq:loss_gen}.
Extra performance gain can be obtained by adding the policy-gradient updates via the Gumbel-softmax trick (GS) discussed in \Secref{sec:main_gs}.
Indeed, GS improves both the plain \rewardnet and \rewardmle models.
This shows the efficacy of directly optimizing the response-generation model \wrt~the learned reward function.
Further discussion is provided in \Secref{sec:exp_abla}.
% \yy{people may have questions that when we add gs, the performance boosted but rewardnet is better than rewardmle, contradictory with previous observation}

Appendix~\ref{sec:exp_galaxy} provides the experimental results when applying our method onto the recent  GALAXY backbone \citep{he2022galaxy}.
Appendix~\ref{sec:exp_multiwoz21} discusses the results on the MultiWOZ 2.1 dataset.

\myparagraph{Low-resource experiment.}
We evaluate our method on the low-data regime by following the testing strategy in \citet{mintl2020}.
Specifically, we use $5\%$, $10\%$, and $20\%$ of the training data to train our basic \rewardnet and \rewardmle models in Table~\ref{table:main}, without the GS component. 
We compare them with the baseline scores in \citet{mintl2020}.
Table~\ref{table:low_resource} reports the results.
It is clear that our models outperform the baselines, MinTL and DAMD, showing the efficacy of our method.
Compared with Table~\ref{table:main}, our models trained with $20\%$ of the data perform competitively with the baseline methods trained on the full training set.

\begin{table}[tb] 
\vspace{-2mm}
\captionsetup{font=small}
\caption{
\footnotesize{Results on the simulated low-resource settings, where $5\%$, $10\%$, and $20\%$ of the training data is used to train the models.
The best result on each metric under each setting is bold.
``Comb." is the Combined Score.
All our provided results are the average over five random seeds.
Baseline results are from \citet{mintl2020}.}
} 
\label{table:low_resource} 
\vspace{-.7em}
\centering 
% \def\arraystretch{1.2}
\resizebox{1.\textwidth}{!}{
\begin{tabular}{@{}ccccccccccccc@{}}
\toprule
\multirow{2}{*}{Model}     & \multicolumn{4}{c}{$5\%$}                              & \multicolumn{4}{c}{$10\%$}                            & \multicolumn{4}{c}{$20\%$}       \\
                           & Inform & Success & BLEU  & Comb.                      & Inform & Success & BLEU  & Comb.                      & Inform & Success & BLEU  & Comb. \\ \midrule
\multicolumn{1}{c|}{DAMD}  & 56.60  & 24.50   & 10.60 & \multicolumn{1}{c|}{51.15} & 62.00  & 39.40   & 14.50 & \multicolumn{1}{c|}{65.20}  & 68.30  & 42.90   & 11.80 & 67.40 \\
\multicolumn{1}{c|}{MinTL} & 75.48  & 60.96   & 13.98 & \multicolumn{1}{c|}{82.20}  & 78.08  & 66.87   & \textbf{15.46} & \multicolumn{1}{c|}{87.94} & 82.48  & 68.57   & 13.00 & 88.53 \\
\multicolumn{1}{c|}{\rewardnet:3} & 81.22  & 67.37   & 12.82 & \multicolumn{1}{c|}{87.11}  &   \textbf{92.39} & \textbf{78.98}   & 13.36 & \multicolumn{1}{c|}{\textbf{99.05}} & 89.83  &  \textbf{79.30}  & 15.18 & 99.75 \\
\multicolumn{1}{c|}{\rewardmle:5} & \textbf{82.90}  & \textbf{69.61}   & \textbf{14.26} & \multicolumn{1}{c|}{\textbf{90.51}}  & 89.67   &  77.48  & 14.80 & \multicolumn{1}{c|}{98.38} & \textbf{90.15}  &  78.70  & \textbf{15.81} & \textbf{100.24} \\
\bottomrule
\end{tabular}
}
\vspace{-1.0em}
\end{table}

\vspace{-.6em}
\subsection{Ablation Study} \label{sec:exp_abla}
\vspace{-.4em}
The ablation study considers the following four research questions to better understand our methods.

\textbf{(a):}~\textit{What if we learn the reward function via a different number of trajectories?}
In Fig.~\ref{fig:listnet_p1_num_traj} and \ref{fig:listmle_smax_num_traj}, we vary the number of trajectories used for the reward-learning losses in Table~\ref{table:main}.
To avoid unwanted interference, we use the basic version of models without the GS component.
The case of using two trajectories reduces to the pairwise-preference loss discussed in \Secref{sec:background}.

As shown in Fig.~\ref{fig:listnet_p1_num_traj} and \ref{fig:listmle_smax_num_traj}, our generalized approach of using multiple trajectories to learn the reward function provides the flexibility to outperform the classical pairwise-preference learning.
This is more apparent in the \rewardmle models, which are less sensitive to small errors in the ground-truth scores. 
In general, the optimal trajectory number may depend on the scoring quality.

\begin{figure}[tb]
     % \vspace{+2mm}
     \centering
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./Tex/fig/ListNet_p=1_line.pdf}
         \captionsetup{font=small}
         \vspace{-6mm}
         \caption{\rewardnet}
         \label{fig:listnet_p1_num_traj}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./Tex/fig/listMLE_softmax_line.pdf}
         \captionsetup{font=small}
         \vspace{-6mm}
         \caption{\rewardmle}
         \label{fig:listmle_smax_num_traj}
     \end{subfigure}
     \hfill
    %  \rulesep
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./Tex/fig/listNet_3_line.pdf}
         \captionsetup{font=small}
         \vspace{-6mm}
         \caption{\rewardnet}
         \label{fig:listnet_3_transf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./Tex/fig/ListMLE_5_line.pdf}
         \captionsetup{font=small}
         \vspace{-6mm}
         \caption{\rewardmle}
         \label{fig:listmle_5_transf}
     \end{subfigure}
     \vspace{-2mm}
     \captionsetup{font=small}
        \caption{ 
        \footnotesize{Line plots comparing the Combined Score when the \rewardnet and \rewardmle losses are constructed under a different number of sampled trajectories or different probabilistic transforms.
        The $y$-axis represents the Combined Score.
        $p=1,2,3,4$ is the escort transform with power $1,2,3,4$.
        ``smax" is the softmax transform.
        Results are the average over five random seeds.}
        }
        \label{fig:abla_sweep}
        \vspace{-1.5em}
\end{figure}

\textbf{(b):}~\textit{Do different probabilistic transforms in reward learning objectives affect the performance?}
We modify the basic version of the \rewardnet and \rewardmle models in Table~\ref{table:main} by using the softmax transform and by using different powers in the escort transform in the reward learning losses Eqs.~\eqref{eq:listnet} and \eqref{eq:listmle}.
For the escort transform, we consider $\Phi=(\cdot)^p, p\in \cbr{1,2,3,4}$.

Figs.~\ref{fig:listnet_3_transf} and \ref{fig:listmle_5_transf} plot the resulting Combined Scores.
We see that the \rewardmle model is less sensitive to the choice of probabilistic transform --- all the considered variants have a Combined Score of at least $104$.
In fact, changing its softmax transform used in Table~\ref{table:main} to the escort transform with power two improves the performance to $106.77$.
Thus, the choice of probabilistic transform provides an additional angle to improve the learned reward function and the entire ToD model.

\begin{figure}[tb]
     \vspace{-2mm}
     \centering
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./Tex/fig/comb_alpha_line.pdf}
         \captionsetup{font=small}
         \vspace{-6mm}
         \caption{\footnotesize{Combined Score}}
         \label{fig:vary_alpha_comb}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./Tex/fig/inform_alpha_line.pdf}
         \captionsetup{font=small}
         \vspace{-6mm}
         \caption{\footnotesize{Inform Rate}}
         \label{fig:vary_alpha_inform}
     \end{subfigure}
     \hfill
    %  \rulesep
    \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./Tex/fig/success_alpha_line.pdf}
         \captionsetup{font=small}
         \vspace{-6mm}
         \caption{\footnotesize{Success Rate}}
         \label{fig:vary_alpha_success}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./Tex/fig/bleu_alpha_line.pdf}
         \captionsetup{font=small}
         \vspace{-6mm}
         \caption{\footnotesize{BLEU Score}}
         \label{fig:vary_alpha_bleu}
     \end{subfigure}
     \vspace{-3mm}
     \captionsetup{font=small}
        \caption{ 
        Line plots showing the four automatic evaluation metrics of the \rewardnet + GS model in Table~\ref{table:main} under different $\alpha$ values in the generation-model loss Eq.~\eqref{eq:loss_gen}.
        Results are the average over five seeds.
        }
        \label{fig:vary_alpha}
        \vspace{-5mm}
\end{figure}

\textbf{(c):}~\textit{Is our method sensitive to the coefficient $\alpha$ in the generation-model loss Eq.~\eqref{eq:loss_gen}?}
To investigate the robustness of our method under different weights for the policy-gradient optimization of the response-generation model.
We select our best policy-gradient-based model in Table~\ref{table:main}, the \rewardnet + GS model, and vary the $\alpha$ coefficient in the generation-model loss Eq.~\eqref{eq:loss_gen}.
Fig.~\ref{fig:vary_alpha} plots the resulting four automatic evaluation metrics.

We see that our model is relatively robust to the choice of $\alpha$.
The five variants in Fig.~\ref{fig:vary_alpha} all have Combined Scores of at least $105$, higher than the best baseline result of $104.78$ in Table~\ref{table:main}.
In fact, by changing the $\alpha$ coefficient  to $0.5$ from $0.1$ used in Table~\ref{table:main}, we achieve a \emph{even better} Combined Score of $\approx 107.2$.
Further, the capability of task completion and the fluency of the generated responses are both relatively insensitive to the choice of $\alpha$.

\textbf{(d):}~\textit{How does the addition of the policy-gradient method Gumbel-softmax help the performance?}
Fig.~\ref{fig:abla_gs} compares the performance of our models in Table~\ref{table:main}, with error bars showing the standard deviation of the Combined Score over five seeds.
It is clear that the addition of the Gumbel-softmax method can not only improve the score but also reduce the performance variation, which is apparent when comparing the \rewardmle model with the \rewardmle + GS model.

As discussed in \Secref{sec:main_gs}, the Gumbel-softmax (GS) trick can be more advantageous than the classical REINFORCE method \citep{reinforce1992} for the policy-gradient update.
As a demonstration, we conduct a toy experiment following \citet{arsm2019} and plot the results in Fig.~\ref{fig:abla_toy}.
The task here is to learn the parameter $\vpsi$ of a $D$-dimensional categorical distribution to maximize a simple reward function.
Specifically, denote the sigmoid function as $\sigma(\cdot)$, the goal is
\begin{equation*}\textstyle
    \max_{\vpsi \in \R^D} \E_{x \sim \mathrm{Cate}(\sigma(\vpsi))}\sbr{f(x)},\quad f(x) \triangleq 0.5 + x / (D \cdot R),\; \forall\, x \in \cbr{1, \ldots, D}, 
\end{equation*}
where $\mathrm{Cate}(\sigma(\vpsi))$ denotes the categorical distribution with probability vector $\sigma(\vpsi)$, and $D=R=30$.
The best $\sigma(\vpsi)$ is $(0,\ldots,0,1)$, leading to the optimal expected reward of $\approx 0.533$.
We initialize $\vpsi = \vzero$ and use one sample for the stochastic gradient-ascent update, with a learning rate of $1.0$.

The first row of Fig.~\ref{fig:abla_toy} traces the objective function during the training process when using the true gradient, REINFORCE, and the GS for policy-gradient updates.
We see that the REINFORCE method converges to a local maximum, while the GS method reaches the global optimum, as using the true gradient for updates.
The second row shows the gradients for $\theta_1$ and $\theta_D$, where we see that gradient estimates from the REINFORCE method are both unstable and vanishing, compared to the GS method.
The learned probabilities $\cbr{\sigma(\vpsi)_1, \ldots, \sigma(\vpsi)_D}$ is traced in the third row, where the red line is for $\sigma(\vpsi)_D$ that should ideally be $1$, and the shadowed lines are for the other components that ought to be $0$.
The learning process of the GS method closely resembles that of using the true gradient, while REINFORCE oscillates around a local optimum.
The last row of Fig.~\ref{fig:abla_toy} plots the estimate of gradient variance via $500$ samples, averaged over each component of the $\vpsi$ vector.
The gradient variance of the REINFORCE method is on the order of $10^{-2}$ at the beginning and converges to roughly $10^{-4}$, while the GS is $10^{-6}$ throughout the training process.
This toy experiment shows that a low-variance method, such as the GS, can be critical to the success of policy-gradient training.




\begin{figure}[tb]
\vspace{-2mm}
    \centering
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{./Tex/fig/w_wo_gs_bar.pdf}
        \captionsetup{font=small}
        \vspace{-2em}
        \caption{\footnotesize{ Bar plot comparing our four models in Table~\ref{table:main}.
        Mean and one standard deviation over five random seeds are shown.
        ``R-Net" denotes \rewardnet. ``R-MLE" is \rewardmle. ``GS" is Gumbel-softmax.
        }}
        \label{fig:abla_gs}
    \end{minipage}
    \hfill
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{./Tex/fig/gs_gradient_var_plot.pdf} % figsize=(9, 6)
        \captionsetup{font=small}
        \vspace{-2em}
        \caption{\footnotesize{Toy experiment comparing REINFORCE and Gumbel-softmax in reward maximization, the estimated gradients, the estimated probabilities, and the gradient variance.
        See \Secref{sec:exp_abla} for details.}}
        \label{fig:abla_toy}
    \end{minipage}
    \vspace{-.8em}
\end{figure}




\begin{figure}[tb]
    \centering
    \begin{minipage}{0.49\textwidth}
        \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./Tex/fig/appropriate_bar.pdf}
         \captionsetup{font=small}
         \vspace{-6mm}
         \caption{Appropriateness}
         \label{fig:appropriate}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./Tex/fig/fluency_bar.pdf}
         \captionsetup{font=small}
         \vspace{-6mm}
         \caption{Fluency}
         \label{fig:fluency}
     \end{subfigure}
     \vspace{-3mm}
     \captionsetup{font=small}
        \caption{ 
        \footnotesize{Bar plots for the results of human evaluation on appropriateness and fluency, showing the mean and one standard deviation of each method. 
        The scores are on a $5$ scale and higher scores indicate better results.
        ``GPT-C" denotes GPT-Critic.
        Details for the setup of human evaluation are discussed in \Secref{sec:exp_further}.}
        }
        \label{fig:human_eval}
    \end{minipage}
    \hfill
    \begin{minipage}{0.49\textwidth}
        \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./Tex/fig/joint_acc_bar.pdf}
         \captionsetup{font=small}
         \vspace{-6mm}
         \caption{Joint Accuracy}
         \label{fig:dst_joint_acc}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./Tex/fig/slot_acc_bar.pdf}
         \captionsetup{font=small}
         \vspace{-6mm}
         \caption{Slot Accuracy}
         \label{fig:dst_slot_acc}
     \end{subfigure}
     \vspace{-3mm}
     \captionsetup{font=small}
        \caption{ 
       \footnotesize{ Bar plots for the quality of the generated dialogue states, showing the mean and standard deviation of two metrics.
        ``GPT-C" denotes GPT-Critic, ``R-Net" denotes \rewardnet, ``R-MLE" is \rewardmle.
        The results of UBAR and GPT-Critic are from \citet{gptcritic2022}.
        Our results are over five random seeds.}
        }
        \label{fig:further_dst}
    \end{minipage}
    \vspace{-1.2em}
\end{figure}




\vspace{-.5em}
\subsection{Further Analysis} \label{sec:exp_further}
\vspace{-.5em}

\myparagraph{Human evaluation.}
For a more comprehensive evaluation of our method, we conduct a human evaluation on the quality of the generated responses, where our model and the top two baselines in Table~\ref{table:main}, GPT-Critic and CASPI, are compared.
We follow the evaluation protocol in prior work \citep[\eg,][]{damd2020,caspi2021,gptcritic2022} to evaluate on two metrics:
1) \textbf{Appropriateness}: measures the appropriateness of the generated response under the context of the dialogue turn;
2) \textbf{Fluency}: evaluates the comprehensibility and coherency of the generated response.
We randomly picked $50$ turns in the test set and showed to $10$ evaluators the responses generated from each method, together with the dialogue history up to that turn.  
The method names were anonymized.
The evaluators were asked to read the dialogue history and score the response on a $5$-Point Likert Scale $\cbr{1,2,3,4,5}$, where score $5$ is the highest and $1$ the lowest.

Fig.~\ref{fig:human_eval} summarizes the evaluation results.
We see that our model outperforms the baselines in both the appropriateness and fluency scores.
The human-evaluation results coincide with our comparatively good dialogue-task completion and BLEU score in
Table~\ref{table:main}.

\myparagraph{Examples of the generated dialogues.}
Tables~\ref{table:dia_pmul4610} and \ref{table:dia_sng1012} in Appendix~\ref{sec:appendix_example} conduct two case studies comparing the generated responses from our method with those from the baselines GPT-Critic and CASPI.
We additionally annotate the generated responses to discuss the quality of those generations.
These examples show that the responses from our model compare favorably with the baselines in both task completion and comprehensibility, aligning with the automatic and human evaluations.

\myparagraph{Quality of the DST.}
To further understand the performance gain of our models, we compare our basic \rewardnet and \rewardmle models in Table~\ref{table:main} with the baselines UBAR and GPT-Critic on the quality of the generated dialogue states.
Fig.~\ref{fig:further_dst} plots the results of the dialogue state prediction, measured by the two metrics Joint (Goal) Accuracy and Slot Accuracy \citep{wu2019transferable}.
We see that our two models have more accurate DST than the two baselines, which can be related to their better performance in Table~\ref{table:main}.
Interestingly, the DST of the \rewardmle model is also better than that of the \rewardnet model. 
This may suggest that a better reward model not only benefits the learning of response generation, but also the DST. 
These two losses are jointly minimized in training the ToD model, and thus a good response-generation loss from a better reward model may help the optimization of the DST loss.




==> Reward Learning for Dialogs (ICLR 2023)/Tex/method.tex <==
\vspace{-.2em}
\section{Main Method}\label{sec:main_method}
\vspace{-.2em}
In this section, we first introduce two objectives for reward-function learning
based on the classical approaches in the learning-to-rank (LTR) literature \citep{liu2009learning}.
Then we use MinTL \citep{mintl2020} as an example to demonstrate how we can use the learned reward function as a plugin module to improve existing methods of training the E2E ToD models.

% \subsection{Overview of the Training Process}\label{sec:method_overview}
% \st{TODO: @yihao describe the training process, how we get multiple alternative dialogue trajectories, and how to rank them (call the score s)}
\vspace{-.4em}
\subsection{Two Generalized Objectives for Reward Learning}\label{sec:main_rew_obj}
\vspace{-.4em}
%Instead of learning the reward function $\gR_{\theta}(o_t, a_t, g)$ via the pairwise preference learning, 
We introduce two objectives, \texttt{RewardNet} and \texttt{RewardMLE}, both of which can utilize multiple dialogue trajectories 
on each update for optimizing the reward function.
Our motivation is that, compared with the pairwise approach described in Eq.~\eqref{eq:original_pref_rew}, these two objectives consider more information at each training step, and thus can be more effective for reward learning and may lead to a better solution under the stochastic training setting.
% , these two objectives can improve efficiency of the reward learning, especially under the stochastic training settings.

\myparagraph{Setup.}
Assume that there are $N \geq 2$ dialogue trajectories, denoted by $\gD_{N} \triangleq (\tau_1, \tau_2, \ldots, \tau_N)$, 
and each trajectory $\tau_i$ has an automatic evaluation score $S(\tau_i)$.\footnote{We use the \texttt{Combined Score} \citep{sfnrl2019} as $S(\tau_i)$. Detailed definition is delayed to \Secref{sec:exp}.}
For simplicity, we assume that these $N$ dialogue trajectories are of equal length $T$ and are already sorted by the automatic evaluation scores, \ie, $ \tau_1 \succ \tau_2 \succ \cdots \succ \tau_N$, or equivalently, $S(\tau_1) > S(\tau_2) > \cdots > S(\tau_N)$.
We denote the accumulated reward of dialogue trajectory $\tau_i$ from $\gR_\theta$ as $J(\tau_i; \theta)= \sum_{t=0}^{T}\gR_{\theta}(o_t^{(i)},a_t^{(i)}, g^{(i)})$.
Our goal is to learn a reward function $\gR_{\theta}(o, a, g)$ such that the accumulated rewards of those trajectories can reflect the ranking order, \ie, 
$J(\tau_1; \theta) > \cdots > J(\tau_N; \theta)$. 

\myparagraph{\texttt{RewardNet}.}
The proposed \texttt{RewardNet} objective for reward function learning is adapted from the \textit{ListNet} loss \citep{listnet2007} in the LTR literature. 
Specifically, given $N$ trajectories and their associated scores, we 
define the \texttt{RewardNet} loss as the cross entropy between $\{J(\tau_i; \theta)\}_{i=1}^{N}$ and $\{S(\tau_i)\}_{i=1}^{N}$:
% \begin{align}\textstyle
%     \ell_{\texttt{RewardNet}}(\theta; \gD_{N} ) \triangleq& - \sum_{i=1}^{N} P_{S}(\tau_i)\cdot \log\left( P_{J(\tau ; \theta)}(\tau_i)\right)\,, \label{eq:listnet}\\ 
%     \text{with} ~~~~~ P_{S}(\tau_i) = {S(\tau_i)} \bigg/ {\sum_{k=1}^{N} S(\tau_k)} ,&~~~~ P_{J(\tau ; \theta)}(\tau_i) = \Phi(J(\tau_i; \theta)) \bigg/ \sum_{k=1}^{N}\Phi(J(\tau_k; \theta)) \,, \notag 
% \end{align}
\begin{equation}\label{eq:listnet}\textstyle
\resizebox{.53\linewidth}{!}{%
$
   \ell_{\texttt{RewardNet}}(\theta; \gD_{N} ) \triangleq - \sum_{i=1}^{N} P_{S}(\tau_i)\cdot \log\left( P_{J(\tau ; \theta)}(\tau_i)\right)\,,
    $%    
}
\end{equation}
\text{with}
\begin{equation*}
\resizebox{.82\linewidth}{!}{%
$
   P_{S}(\tau_i) = {S(\tau_i)} \big/ \big({\sum_{k=1}^{N} S(\tau_k)}\big),~~~~ P_{J(\tau ; \theta)}(\tau_i) = {\Phi(J(\tau_i; \theta))}\big/ \big(\sum_{k=1}^{N}\Phi(J(\tau_k; \theta))\big)\,,
    $%    
}
\end{equation*}
where $\Phi(\cdot)$ is a monotonic positive function defined on $\mathbb{R}^{+}$, 
%which can be either identity or exponential functions.
and $P_{S}(\tau_i)$ is a normalized probability vector defined by the true evaluation scores of those $N$ trajectories. 
%\yy{ normalized  probability of dialogue trajectory $\tau_i$ (not sure?)}\st{normalized prob. defined by the true score of each trajectory, similar to Eq. 5 of the CASPI paper.}.  
Note that when $N=2$ and $\Phi$ is the identity function, \rewardnet can be viewed as a \textit{soft} version of the pairwise preference loss defined in Eq.~\eqref{eq:original_pref_rew}, where the hard binary preference labels are replaced by $\{P_{S}(\tau_i)\}_{i=1}^{N}$. 
This soft pairwise loss is adopted for reward learning in the recent CASPI paper \citep{caspi2021}.
%Besides, this special pairwise loss is also utilized in CASPI \citep{caspi2021}.
%Note that the pairwise loss proposed in CASPI \citep{caspi2021} can be viewed as a special case of \texttt{RewardNet} loss where the number of trajectories $N=2$ \st{and when $\Phi$ is the identity function}.


\myparagraph{\texttt{RewardMLE}.}
The \texttt{RewardMLE} objective is based on the \textit{ListMLE} loss \citep{listmle2008}, 
where we only utilize the ranking order in the batched dialogue trajectories $\gD_{N} $, rather than the original metric scores $\{S(\tau_i)\}_{i=1}^{N}$. 
Let $y = \mathrm{rank}(S)$ be the random variable that represents the ranking order of the dialogue trajectories ($y(\tau_i) = i, \forall\, i$, if the batched trajectories $\gD_{N}$ are sorted). 
The \texttt{RewardMLE} objective is defined as the negative log-likelihood of the ranking order $y$ under the Plackett-Luce choice model \citep{plackett1975analysis,luce2012individual} induced by the accumulated reward of each trajectory $\{J(\tau_i; \theta) \}_{i=1}^N$.
Specifically, the loss is defined as
% \begin{align}
%     \ell_{\texttt{RewardMLE}}(\theta; \gD_{N}) &\triangleq -\log P\br{y \given \{J(\tau_i; \theta)\}_{i=1}^{N}}\,, \label{eq:listmle}\\
%     \text{with}~~~~~~ P\br{y\given \{J(\tau_i; \theta)\}_{i=1}^{N}} &= \prod_{\textcolor{blue}{i=1}}^{N} \cbr{\Phi(J(\tau_i; \theta)) \bigg/ \sum_{\textcolor{blue}{k=i}}^{N}\Phi(J(\tau_k ; \theta))} \,, \notag 
% \end{align}
\begin{equation}\label{eq:listmle}\textstyle
\resizebox{.5\linewidth}{!}{%
$
  \ell_{\texttt{RewardMLE}}(\theta; \gD_{N}) \triangleq -\log P\br{y \given \{J(\tau_i; \theta)\}_{i=1}^{N}}\,,
    $%    
}
\end{equation}
with
\begin{equation*}
\resizebox{.61\linewidth}{!}{%
$
   ~~~~~~ P\br{y\given \{J(\tau_i; \theta)\}_{i=1}^{N}} = \prod_{\textcolor{blue}{i=1}}^{N} \cbr{\Phi(J(\tau_i; \theta)) \big/ \sum_{\textcolor{blue}{k=i}}^{N}\Phi(J(\tau_k ; \theta))} \,,
    $%    
}
\end{equation*}
where trajectories in $\gD_{N}$ are assumed sorted as described in the problem setup, \ie, $\tau_1 \succ \cdots \succ \tau_N$. 
Since \texttt{RewardMLE} only requires the ranking information derived from the raw scores,
it is potentially a more robust choice when the preference scores could be inaccurate.
%the ranking orders of the preference scores are favored.
%\st{
%\texttt{RewardMLE} only uses the ranking information derived from the raw scores, rather than the numerical scores themselves, it is potentially more robust than %\texttt{RewardNet} to the small inaccuracies in the raw scores.
%Such inaccuracies may be inevitable since the scores come from non-human-expert automatic evaluation.
%}
%\yy{@shentao, and add intuition why to use listMLe}


%As discussed in \Secref{sec:method_overview}, 
%each ground-truth dialogue trajectory is associated with multiple alternatives.
% The preference amount them naturally leads to a listwise ranking problem \citep{liu2009learning}, rather than the pairwise preference discussed in \Secref{sec:rew_from_pref}.
% Therefore, we extend the pairwise-preference loss for reward learning Eq.~\eqref{eq:original_pref_rew} to the case of $n \geq 3$ trajectories, by adapting it with the listwise ranking losses in the learning-to-rank (LTR) literature.
% In this work, we consider two classical listwise ranking losses ListNet loss \citep{listnet2007} and ListMLE loss \citep{listmle2008}.

% \yy{r does not depend on h, this is  slightly different, it only depends on $o_t, a_t, g$}

% \st{@yihao do we also need to change $\hat r$  in Section 2.2 to depend on $o_t$ ???}

% \st{@yihao double check whether the input to $\hat{r}$ is $o_t$ or $h_t$ ???}

% Assume that there are in total $n$ trajectories including the ground-truth one, and denote the $n$ trajectories as $\br{h_T^1, \ldots, h_T^n}$, with associated scores $s=\br{s_1, \ldots, s_n}$ as discussed in xx.
% %\Secref{sec:method_overview}.
% Similar to the goal of LTR, we learn the reward function $\hat r\br{o,a,g;\theta} \in [0,1]$ such that the ranking of the $n$ trajectories resembles the ranking of the true scores, where the trajectories are ranked by the sum of rewards.
% For notation simplicity, we denote $\hat r(h_T^j;\theta) = \sum_{ \br{o_t, a_t}\in h_T^j } \hat r\br{o_t, a_t, g;\theta}, \forall\, j=1,\ldots,n$, where $g$ is the common goal of these $n$ trajectories.
 
% Let $f$ be an increasing and positive function on $\R_{\geq 0}$. 
% The ListNet loss is defined as the cross entropy of the two score lists $\{\hat r(h_T^j;\theta)\}_{j=1}^n$ and $s$, \ie, 
% \begin{equation}\label{eq:listnet}
% \resizebox{.94\textwidth}{!}{%
% $
%     \gL_{\mathrm{ListNet}}\br{\theta; \{\hat r(h_T^j;\theta)\}, s} = -\sum_{i=1}^n P_{s}(i) \cdot \log\br{P_{\{\hat r(h_T^j;\theta)\}}(i)}, P_{\{\hat r(h_T^j;\theta)\}}(i) = \frac{f(\hat r(h^i_T;\theta))}{\sum_{k=1}^n f(\hat r(h^k_T;\theta))},
%     $%    
% }
% \end{equation}
% and similarly for $P_s(i)$.
% In the ListMLE loss, the ranking of the scores $ y = \mathrm{rank}(s)$ is used instead of the original scores $s$.
% The loss is defined as the negative log-likelihood of $y$ under the Plackett-Luce choice model \citep{plackett1975analysis,luce2012individual} induced by the scores $\{\hat r(h_T^j;\theta)\}_{j=1}^n$, \ie,
% \begin{equation}\label{eq:listmle}
% \resizebox{.94\textwidth}{!}{%
% $
%     \gL_{\mathrm{ListMLE}}\br{\theta; \{\hat r(h_T^j;\theta)\}, y} = -\log P\br{y \given \{\hat r(h_T^j;\theta)\}}, P\br{y \given \{\hat r(h_T^j;\theta)\}} = \prod_{i=1}^n \frac{f\br{ \hat r\br{h_T^{y(i)};\theta} }}{\sum_{k=i}^n f\br{\hat r\br{h^{y(k)}_T;\theta}}},
%     $%    
% }
% \end{equation}
% where $y(i)$ is the index of item that is ranked at the position $i$ and similarly for $y(k)$.
In Eqs.~\eqref{eq:listnet} and \eqref{eq:listmle}, the monotonic positive function $\Phi$ transforms the unnormalized inputs $\{J(\tau_i; \theta)\}_{i=1}^{N}$ to a $N$-dimensional probabilistic simplex.
In this work, we consider $\Phi$ being exponential function $\exp(\cdot)$ and power function $(\cdot)^p, p\in \mathbb{N}$, which are respectively known as the softmax transform and the escort transform \citep{escort2020}.

\vspace{-.4em}
\subsection{Policy Gradient Update with Learned Reward Function}\label{sec:main_gs}
\vspace{-.4em}
With the learned reward function $\gR_{\theta}(o, a, g)$, the next step is to improve the parametrized dialogue agents $\pi_{\phi}$ via policy gradient methods \citep{rlintro2018}, given a collected offline dataset $\hat{\mathsf{D}} := \{\tau_{k}\}_{k=1}^{K}$.
A classical approach to train the policy $\pi_{\phi}$ is to estimate the policy gradient via the REINFORCE method \citep{reinforce1992}:
\begin{align}\textstyle
\nabla_{\phi}J_{\small{\mathrm{REINFORCE}}}(\pi_{\phi}) = \E_{ (g, h_t) \sim \hat{\mathsf{D}}, \tilde{a}_{t} \sim \pi_\phi(\cdot \given h_t)}[\nabla_{\phi}\log \pi_{\phi}(\tilde{a}_{t} \given h_t)\cdot G^{\pi_{\phi}}(h_t , \tilde{a}_{t},g)]\,, \label{eq:pg_reinforce}
\end{align}
where $G^{\pi_{\phi}}(h_t , \tilde{a}_{t},g)$ is the (discounted) accumulated reward that the agent  $\pi_{\phi}$ receives, starting from the observation $o_t$ (part of $h_t$) and action $\tilde{a}_{t}$, under the given goal $g$. 
%Previous work \citep{caspi2021} indicates that 
When the discount factor $\gamma > 0$, estimating $G^{\pi_{\phi}}(h_t, \tilde{a}_{t},g)$ requires Monte Carlo sampling (on-policy) or temporal difference learning (off-policy), both of which require learning an additional value-function network.
Empirically we observe that learning an additional action-value function could introduce  instability and extra compute to the subsequent training of the E2E dialogue model.
To simplify the training pipeline, we simply set the discount factor $\gamma = 0$, and thus $G^{\pi_{\phi}}(h_t, \tilde{a}_{t},g) = \gR_{\theta}(o_t, \tilde{a}_t, g)$. 

Though the policy gradient estimator defined in Eq.~\eqref{eq:pg_reinforce} is unbiased, 
it tends to have high variance, especially when the action space is large.
Unfortunately, in the E2E ToD system, the action space is often defined to be the Cartesian product of the vocabulary, which itself has a dimension larger than $30000$.
As a result, optimizing the agent $\pi_{\phi}$ by the REINFORCE estimator may suffer from divergent training.
%the policy optimization with the REINFORCE method may be inefficient or even diverge. 
We illustrate this phenomenon via a toy example in \Secref{sec:exp_abla}.

To mitigate the high-variance issue of the REINFORCE estimator, we utilize the Gumbel-softmax (GS) trick \citep{jang2016categorical,maddison2016concrete, fan2021contextual} to reduce the variance. 
Specifically,
\begin{align}\textstyle
J_{\tiny{\mathrm{GS}}}(\pi_{\phi}) &= \E_{a_t \sim  \pi_\phi(\cdot \given h_t)}[\gR_{\theta}(o_t, a_t, g)]
\notag \approx \E_{\pmb{\epsilon} \sim \mathrm{Gumbel}(0, 1)}[\gR_{\theta}(o_t,f_{\phi}(h_t, \pmb{\epsilon}) , g)]\,, \label{equ:gs_estimator}
\end{align} 
% $$
% f_{\phi}(h_t, \pmb{\epsilon})= \sbr{f_{\phi}^{(1)}(h_t, \pmb{\epsilon}), \ldots, f_{\phi}^{(|\sA|)}(h_t, \pmb{\epsilon})} \in \mathbb{R}^{|\sA|},~~~\text{and}~~~f_{\phi}^{(i)}(h_t, \pmb{\epsilon}) = \frac{\exp((l_i(h_t; \phi) + \epsilon_i) / \lambda)}{\sum_{j=1}^{|\sA|} \exp((l_j(h_t; \phi) + \epsilon_j) / \lambda)}\,,
% $$
\begin{equation*}
\resizebox{.90\linewidth}{!}{%
$
  \text{with}~~~~ f_{\phi}(h_t, \pmb{\epsilon})= \sbr{f_{\phi}^{(1)}(h_t, \pmb{\epsilon}), \ldots, f_{\phi}^{(|\sA|)}(h_t, \pmb{\epsilon})} \in \mathbb{R}^{|\sA|},~~~\text{and}~~~f_{\phi}^{(i)}(h_t, \pmb{\epsilon}) = \frac{\exp((l_i(h_t; \phi) + \epsilon_i) / \lambda)}{\sum_{j=1}^{|\sA|} \exp((l_j(h_t; \phi) + \epsilon_j) / \lambda)}\,,
    $%    
}
\end{equation*}
where $\{l_{i}(h_t; \phi)\}_{i=1}^{|\sA|}$ are the logits of the categorical distribution defined by the agent $\pi_{\phi}$, and $\lambda$ is the temperature parameter that we set as 1.
Besides, following the pessimistic principle in offline RL \citep{buckman2020importance}, 
we add a weighted regularization such that the actions generated by the agent $\pi_{\phi}$ are close to the actions in the dataset $\hat{\mathsf{D}}$,
\begin{align*}\textstyle
\ell_\mathrm{W}(\pi_{\phi}) := - \E_{(h_t, a_t,  g) \sim \hat{\mathsf{D}}}[\log \pi_{\phi}(a_t \given  h_t) \cdot \gR_\theta( o_t, a_t, g)] \,,
\end{align*}
which is similar to the weighted behavior cloning in offline RL \citep{wang2020critic}, except that we directly use the intermediate rewards as the weights, rather than using the value function.
Combining the policy gradient and the weighted regularization, we have the following loss for the agent $\pi_{\phi}$:
%The response generation model is updated by both policy gradient and weighted behavior cloning,
\begin{equation}\label{eq:loss_gen} \textstyle
    \ell_{\mathrm{GEN}}(\phi) = -\alpha \cdot J_{\mathrm{GS}}(\pi_{\phi}) +  \ell_\mathrm{W}(\pi_{\phi}) \,,
\end{equation}
where $\alpha$ is the coefficient balancing these two parts.
Note that the original supervised-learning loss of MinTL \citep{mintl2020} can be decomposed into two parts, respectively for the dialogue state tracking (DST)  and the response generation.
We retain the DST loss $\ell_{\mathrm{DST}}(\phi)$ in MinTL and replace its response-generation loss with Eq.~\eqref{eq:loss_gen}.
Our final loss for ToD agent training is
%Combining with the dialogue state tracking (DST) loss as in MinTL \citep{mintl2020}, the final loss for training our E2E ToD system is
\begin{align}
    \ell(\phi) = \ell_{\mathrm{GEN}}(\phi) + \ell_{\mathrm{DST}}(\phi)\,. \label{eq:final_loss}
\end{align}
We illustrate our method in Fig.~\ref{fig:pipeline} and provide an algorithm box in Appendix~\ref{sec:algo_box}.


\begin{figure}[t]
\centering
\vspace{-2mm}
\includegraphics[width=11.5cm]{Tex/fig/Dialogue_flow.PNG}
% \vspace{-1mm}
\captionsetup{font=small}
\caption{Overview of the proposed method. 
% Some notations are labeled along with corresponding components. 
We denote ``Accumulated Reward'' for the learned accumulated reward, 
% ``Automatic Evaluation Score" for the automatic evaluation score of trajectory, 
$J(\cdot;\theta)$ for the accumulated reward of each trajectory, $S(\cdot)$ for the combined score of each trajectory,
% ``DT" the dialogue trajectory.
$\ell_\mathrm{W}$ for the weighted regularization, $\ell_{\mathrm{DST}}$ for the DST loss, 
and ``DH" for the dialogue history.
In the right panel, $(h_t, a_t, g)\sim \hat{\mathsf{D}}$.
We use BART 
% \citep{bart2019} 
for both the reward model and the ToD model.
}
\vspace{-1.5em}
\label{fig:pipeline}
\end{figure}


\myparagraph{Remark}
Eq.~\eqref{eq:final_loss} for the learning of the dialogue agent $\pi_{\phi}$ is essentially a generalized objective from several previous works.
Specifically, if we set $\alpha = 0$ and set the reward function to be constant $\gR_{\theta}(o_t, a_t, g)\equiv 1$, 
 Eq.~\eqref{eq:final_loss} reduces to the objective in MinTL, without any guidance for response-generation from the learned reward function $\gR_{\theta}$.
If we set $\alpha = 0$, and use the \rewardnet loss with $N=2$ and $\Phi=(\cdot)^{1}$ (\ie, the identity function) to train the reward function,  Eq.~\eqref{eq:final_loss} reduces to the objective in CASPI \citep{caspi2021}. 
In \Secref{sec:exp}, we demonstrate the advantages of our  techniques proposed in this section, including the \rewardnet and \rewardmle losses for reward learning, and  the $J_{\mathrm{GS}}(\pi_{\phi})$ for agent training.

% \yy{todo: add some followed up description of behavior policy and data collection}
%\yy{todo: add when we reduce to mintl, and also discussion with caspi.} \st{May be put this on Appendix? Otherwise people may be confused on how we collect the trajectories for reward learning.}

% \yy{todo: need to add some intuition and why we want to use these two loss over pairwise ones}
% \st{I have added some in the paragraph after the heading of Section 3.1}










==> Reward Learning for Dialogs (ICLR 2023)/Tex/related.tex <==
\vspace{-.8em}
\section{Related Work}
\vspace{-.8em}
Recent works on the E2E ToD systems \citep[\eg,][]{wu2019alternating,mintl2020,simpletod2020,ham2020end,soloist2021,ubar2021} have significantly improved the overall system's performance
and simplified the algorithmic designs in earlier works, which require solving several pipeline based sub-tasks \citep[\eg,][]{young2013pomdp,gao2018neural,damd2020}.
%Our approach may provide further enhancement to the original frameworks of E2E modeling.
The reward function trained by our methods can be leveraged as guidance to train existing E2E models, without changing the underlying structures. 
We demonstrate the effectiveness of our proposed reward learning methods under the structure of MinTL \citep{mintl2020} and GALAXY (\citet{he2022galaxy}; in Appendix~\ref{sec:exp_galaxy})
where we only add an additional reward-function-guided objective for the response-generation model, while keeping other components of the respective structure unchanged. 

%\sz{I am a little confused with this sentence: I feel another line of related research should be replaced to One line of. becasue I did not see the contrast between this paragraph and the above paragraph.}
One line of related research is applying RL to train ToD agents.
It is often unsuccessful to directly apply RL algorithms such as the DDPG \citep{lillicrap2015continuous} or PPO \citep{schulman2017proximal} since the agent training could potentially diverge \citep{zhao2019rethinking,gptcritic2022,kwan2022survey}.
Recently, a number of works consider offline RL \citep{offlinetutorial2020} as a promising solution to stabilize the agent training on a static dataset \citep[\eg,][]{jaques2020human,caspi2021,gptcritic2022,verma2022chai,snell2022offline,snell2022context}.
Following the offline RL principle, we use a reward-weighted regularization to stabilize the dialogue-agent training. 
%However, instead of learning an additional Q-function network in previous works \citep[\eg,][]{gptcritic2022,snell2022context},
%we only use the reward function to guide the dialogue-agent training.
Together with the incorporation of the Gumbel-softmax trick to estimate the policy gradient, 
our work retains algorithmic simplicity while improving the training stability and overall performance. 

Finally, 
our paper closely relates to works on reward learning for the ToD systems \citep[\eg,][]{takanobu2019guided,caspi2021}.
This research thread differs from works that directly use a manually designed reward function, 
which only gives sparse signals to indicate whether the agent achieves the goal or not \citep[\eg,][]{weisz2018sample,wu2019switch,gptcritic2022,snell2022context}. 
One line of this research direction is utilizing inverse reinforcement learning (IRL) \citep{russell1998learning} to learn a dense reward function, 
by assuming the collected data be expert demonstrations \citep{takanobu2019guided}. 
%Though using the reward function estimated by IRL allows the dialogue agents to learn faster, especially during the early stage, 
%theoretically the learned dialogue agents can only achieve similar performance with the collected data. 
However, modern IRL techniques such as GAIL-style algorithms \citep{ho2016generative,fu2017learning} often require iterating between reward learning and policy training \citep{finn2016connection}, which is computationally expensive and less scalable to dialogue-generation models.
Besides, the IRL methods aim at justifying the data, while the reward-learning framework in our work seeks to explain the preference among multiple trajectories, potentially leading to \textit{better-than-demo} agents \citep{trex2019,drex2020}.
Our paper is more closely related to the research on reward learning from preferences,
which has recently been adopted in NLP tasks, including training language models \citep{fan2020bayesian, ouyang2022training} and fine-tuning \citep{ziegler2019fine, zhang2021learning, zhang2022allsh},
question-answering with verification \citep{nakano2021webgpt,zhang2021knowing, menick2022teaching, zhang2022passage}, 
and ToD systems \citep{caspi2021}.
These works use the pairwise preference-learning objective in \citet{christiano2017deep}, which can be viewed as a special case of the \texttt{RewardNet} loss discussed in Section~\ref{sec:main_rew_obj}.  
Our work mainly focuses on the ToD task, where we study reward-function learning and reward utilization for training E2E dialogue agents. 
Appendix~\ref{sec:add_related_work} continues the discussion on related reward-learning methods.
%To the best of our knowledge, our in ToD tasks, u.

%in ToD tasks to utilize multiple trajectories to train reward function,
%which could potentially improve the 
%Compared with the pairwise based approaches,
%, \yy{our work can improve the learned reward-function (rewording, I will also discuss this in the main)} and thus the performance of the ToD system.







% \myparagraph{}


==> Reward Learning for Dialogs (ICLR 2023)/Tex/statement.tex <==

\section*{Acknowledgments} 
S. Yang and M. Zhou acknowledge the support of NSF-IIS 2212418 and the Texas Advanced Computing Center (TACC) for providing HPC resources that have contributed to the research results
reported within this paper.

\section*{Ethical Statement} 
We develop our methods based on the publicly available MultiWOZ 2.0 dataset \citep{multiwoz2018}. It is important to note that, like other ToD models, our implementation will likely reflect the socio-economic and entity biases inherent in the MultiWOZ dataset \citep{qian2021annotation}. We initialize model parameters from the pre-trained BART model. 
And a comprehensive analysis of certain biases captured by BART is outside our scope. 
Besides, we invited volunteers for the human evaluation, with transparent and detailed explanations and communications on data usage, research intent, occupied hours, \etc

%  \section{Reproducibility Statement}  

%Example: All of the modeling and training code used for EXT5 and its variants is already open-sourced as a part of the Mesh Tensorflow1 (Shazeer et al., 2018) and T52 (Raffel et al., 2020) Libraries. Addi- tionally, EXMIX is composed of datasets that are already publicly available.

==> Reward Learning for Dialogs (ICLR 2023)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%
\usepackage{amsmath,amsfonts,bm,amsthm,amssymb,mathrsfs,algorithm,algorithmic,url,xcolor}
\usepackage{booktabs,enumitem,multicol,caption,subcaption,pifont,tikz,listings,wrapfig,lipsum,circledsteps,arydshln,hyperref,multirow}
\usepackage{relsize,footnote,makecell}


\hypersetup{
    colorlinks,
    linkcolor={blue!50!black},
    citecolor={blue!50!black},
    urlcolor={red!50!black}
}

\lstset{
    language=Python,
    numberstyle=\tiny,
    mathescape=true, 
    language=Python, 
    columns=fullflexible,
    flexiblecolumns=true,
}

\newcommand{\circled}[1]{\textcircled{\raisebox{-0.9pt}{#1}}}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem} %[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{theorem*}{Theorem}
\newtheorem{claim}{Claim}
\newtheorem{example}{Example}
\newtheorem{fact}{Fact}
\newtheorem{conjecture}{Conjecture}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
\def\eqref#1{(\ref{#1})}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\vpsi{{\bm{\psi}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}





% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


\def\ps{\pmb{s}}
\def\ph{\pmb{h}}
\def\pa{\pmb{a}}
\def\po{\pmb{o}}
\def\pg{\pmb{g}}

\newcommand{\abs}[1]{\left\vert#1\right\rvert}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\br}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\given}{\,|\,}

\newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\denv}{\gD_{\mathrm{env}}}
\newcommand{\dmodel}{\gD_{\mathrm{model}}}


\newcommand{\dbtrue}{d_{\pi_b}^{P^{*}}}
\newcommand{\dpitrue}{d_{\pi}^{P^{*}}}
\newcommand{\dbfake}{d_{\pi_b}^{\widehat{P}}}
\newcommand{\dpifake}{d_{\pi}^{\widehat{P}}}

\newcommand{\dbgtrue}{d_{\pi_b,\gamma}^{P^{*}}}
\newcommand{\dpigtrue}{d_{\pi,\gamma}^{P^{*}}}
\newcommand{\dbgfake}{d_{\pi_b,\gamma}^{\widehat{P}}}
\newcommand{\dpigfake}{d_{\pi,\gamma}^{\widehat{P}}}
\newcommand{\rmax}{r_{\max}}

\newcommand*\diff{\mathop{}\!\mathrm{d}}

\newcommand{\wQ}{{\widehat{Q}}}
\newcommand{\wP}{{\widehat{P}}}
\newcommand{\trueP}{{P^{*}}}

\newcommand*{\defeq}{\stackrel{\mathsmaller{\mathsf{def}}}{=}}

\newcommand{\ie}{\textit{i.e.}}
\newcommand{\eg}{\textit{e.g.}}
\newcommand{\wrt}{\textit{w.r.t.}}
\newcommand{\etc}{\textit{etc.}}
\newcommand{\myparagraph}[1]{\textbf{#1~~}}

\newcommand{\rulesep}{\unskip\ \vrule\ }

\newcommand{\bad}[1]{\hfill \color{Maroon}//~#1}
\newcommand{\good}[1]{\hfill \color{SeaGreen}//~#1}

\newcommand{\rewardnet}{\texttt{RewardNet}~}

\newcommand{\rewardNet}{\texttt{RewardNet}~}

\newcommand{\rewardMLE}{\texttt{RewardMLE}~}

\newcommand{\rewardmle}{\texttt{RewardMLE}~}
